Scalable Estimation of Epidemic Thresholds via Node Sampling

Infectious or contagious diseases can be transmitted from one person to another through social contact networks. In today's interconnected global society, such contagion processes can cause global public health hazards, as exemplified by the ongoing Covid-19 pandemic. It is therefore of great practical relevance to investigate the network trans-mission of contagious diseases from the perspective of statistical inference. An important and widely studied boundary condition for contagion processes over networks is the so-called epidemic threshold. The epidemic threshold plays a key role in determining whether a pathogen introduced into a social contact network will cause an epidemic or die out. In this paper, we investigate epidemic thresholds from the perspective of statistical network inference. We identify two major challenges that are caused by high computational and sampling complexity of the epidemic threshold. We develop two statistically accurate and computationally efficient approximation techniques to address these issues under the Chung-Lu modeling framework. The second approximation, which is based on random walk sampling, further enjoys the advantage of requiring data on a vanishingly small fraction of nodes. We establish theoretical guarantees for both methods and demonstrate their empirical superiority.

==> samplingNewmanTh.tex <==
\section{Estimating the Newman Threshold (Part 4)}
We present a sampling based algorithm to estimate the Newman threshold, i.e. the ratio $\frac{m_2}{m_1}$. 


\begin{algorithm}
\caption{RandomWalkEstimate}\label{alg:rw}
\begin{algorithmic}[1]
\Procedure{Estimate}{$G, r, t^*$}
\label{alg:rwestimate}
\State $x \leftarrow 1.$
\While {$t \le t^* $}
    \State $x \leftarrow $ random neighbor of $x$, chosen uniformly.
\EndWhile
\State $v \leftarrow 0$.
\While{$i \leq r$}
\State $v = v + d_{x}$
\State $x \leftarrow $ random neighbor of $x$, chosen uniformly.
\EndWhile
\State return $v / r$.
\EndProcedure

\end{algorithmic}
\end{algorithm}

Let $G$ be the given graph, with $n$ nodes and $m$ edges. We now show that the above algorithm returns a guaranteed approximation of the Newman threshold. We first state the following easy lemma. Let $\pi$ denote the stationary distribution of the simple random walk on the given graph. Recall that, $\pi$ is given by $\pi_v = \frac{d_v}{\sum_v d_v}$ for all $v$.
For brevity, we define the mixing time of the graph $g$, denoted as $\tmix(G)$, to mean the number of steps required by the simple random walk to reach a distribution $\hat{\pi}$ such that $\|\hat{\pi} - \pi\|_1 = o(\frac{1}{n^2})$.

Let $\vrw$ be the estimate returned by the Algorithm~\ref{alg:rwestimate}. We first show an easy lemma that characterizes the bias of the estimator $\vrw$.
\begin{lemma}
\label{lem:unbiased}
If $x$ is a node that is randomly sampled from $\pi$, and $d_x$ is its degree, then $E[d_x]= \frac{\sum_i d_i^2}{\sum_i d_i}. $ Consequently if $\hat{\pi}$ is such that $\|\pi - \hat{\pi}\|_1 = o(n^{-2})$ and $x$ is sampled from $\hat{\pi}$, then $E[d_x]= (1 \pm o(1))\frac{\sum_i d_i^2}{\sum_i d_i}.$
\end{lemma}

\begin{proof}
It is easy to see that
$$ E_{x\sim \pi} [d_x] = \sum_{v = 1}^{n} d_v \times \pi_v =\frac{\sum_{v} d_v^2}{\sum_v d_v}.$$
We show the second claim as follows: 
$$ |E_{x\sim \pi} [d_x] - E_{x\sim \hat{\pi}} [d_x]| \le  \sum_{v = 1}^{n} d_v  |\pi_v - \hat{\pi_v}| \le n \|\pi - \hat{\pi}\|_1 = o(1).$$

\end{proof}
Next, we show that the estimator $\vrw$ is actually concentrated around its expectation. 

%@article{lezaud1998chernoff, title={Chernoff-type bound for finite Markov chains}, author={Lezaud, Pascal},  journal={Annals of Applied Probability}, pages={849--867}, year={1998}, publisher={JSTOR} }


\begin{theorem} [\cite{lezaud1998chernoff}]
\label{thm:lezaud}
Let $(X_n)$ be a irreducible and reversible Markov Chain on a finite set $V$
with $Q$ being the transition matrix. Let $\pi$ be the stationary distribution.
% Let $(P,\pi)$ be a irreducible and reversible Markov chain on a finite set $V$.
%
Let $f: V\rightarrow \Re$ be such that $E_\pi[f] = 0$, $\|f\|_\infty \leq 1$ and $0 < E_\pi[f^2]\le b^2$. Then, for any initial distribution $q$, any positive integer $r$ and all $0< \gamma \le 1$,

\begin{align*}
  \Pr_q \left[ r^{-1}\sum_{i=1}^r f(X_i)\ge \gamma \right] \le e^{-\varepsilon(Q)/5} S_q \exp\left( -\frac{r\gamma^2\varepsilon(Q)}{4b^2(1 + h(5\gamma/b^2))} \right),
\end{align*}

where $\varepsilon(Q) =1 - \lambda_2(Q)$, $\lambda_2(Q)$ being the second largest eigenvalue of $Q$,  $S_q = \|q/\pi\|_2$ (in the $\ell_2(\pi)$ norm). 

$$ h(x) = \frac{1}{2}(\sqrt{1+x} - (1 - x/2)).$$

If $\gamma \ll b^2$ and $\varepsilon(Q) \ll 1$, the bound is

$$ (1 +o(1))S_q \exp\left( - \frac{r\gamma^2\varepsilon(p)}{4b^2(1+o(1))} \right).$$

\label{thm:markovconc}
\end{theorem}

Using the above result, we bound the sample complexity of our estimator. We first quote the following result that we use to bound $\lambda_1$ of the transition matrix. 

\begin{theorem} Let $\epsilon, \delta\in (0, 1)$. Algorithm~\ref{alg:rwestimate}, using $r = \frac{1}{\varepsilon(P) \epsilon^{3/2}} \times \frac{12m d_{\max}}{(\sum_v d_v^2)} \log(1/\delta)$ and $t^* \ge \tmix(G)$ returns an estimate $\vrw$ that satisfies, with probability $1 - \delta,$
$$ (1 - \epsilon)\frac{\sum_v d_v^2}{\sum_v d_v}\le \vrw \le  (1 + \epsilon)\frac{\sum_v d_v^2}{\sum_v d_v}. $$
The number of nodes that are touched by algorithm is $O(t^{*}  + r)$. 
\end{theorem}
\begin{proof}
In proving the concentration of the estimator $\vrw$, we first look to apply Theorem~\ref{thm:lezaud}. In our setting the set $V$ is the set of vertices and the transition matrix of the random walk is $Q = D^{-1}A$. Recall that $d_{max}$ is the maximum degree of a vertex. 

Define the function $f(X_i)$ as : $$  f(X_i) = d_{\max}^{-1} ( d_{X_i} - E_{\pi}[d_{X_i}]).$$
$f(\cdot)$ clearly satisfies $E_{\pi}[f] = 0$ and that $\|f\|_\infty \le 1$. We can bound $E_{\pi}[f^2]$ as
\begin{align*}
    E_{\pi}[f^2] \le d_{\max}^{-2}E_{\pi}[d_v^2] = d_{\max}^{-2} \sum_v \frac{d_v^2 \times d_v}{2m} =d_{\max}^{-2} \sum_v \frac{d_v^3}{2m} 
\end{align*}


Using the first $t^*$ steps, we reach the distribution $\hat{\pi}$ that satisfies $\|\pi - \hat{\pi}\|_1 = o(n^{-2})$. Hence,
\begin{align*}
    \|\hat{\pi} / \pi\|_2^2 & = \sum_v \pi_v(\hat{\pi}_v/\pi_v)^2 = \sum_v \hat{\pi}_v^2 / \pi_v = \sum_v(\pi_v + (\hat{\pi}_v - \pi_v))^2 / \pi_v\\
    & = \sum_v (\pi_v + 2 (\hat{\pi}_v - \pi_v) + (\hat{\pi}_v - \pi_v)^2/\pi_v)\\
    & = 1 + 2\times (1 - 1) + \sum_v (\hat{\pi}_v - \pi_v)^2/\pi_v \le 1 + \|\pi - \hat{\pi}\|_2^2 / \min(\pi_v)\\
    & \le 1 + \|\pi - \hat{\pi}\|_1^2 (2m/d_{\min})
    = 1 + o(1).
\end{align*}
where the last step follows as $\|\pi - \hat{\pi}\|_1 = o(n^{-2})$.

We use $b^2 = d_{\max}^{-2} \sum_v \frac{d_v^3}{2m}$ and $\gamma = \epsilon d_{\max}^{-1}\times \frac{\sum_v d_v^2}{2m}$. Hence
\begin{align*}
    \gamma / b^2 = \epsilon d_{\max} \frac{\sum_v d_v^2 }{\sum_v d_v^3} \ \mathrm{and}\  
    \gamma^2 / b^2 = \epsilon^2 \frac{(\sum_v d_v^2)^2}{2m (\sum_v d_v^3)}
\end{align*}
Hence,
\begin{align*}
    h(5\gamma / b^2)& = \left( 1 + 5 \epsilon d_{\max} \frac{\sum_v d_v^2 }{\sum_v d_v^3}\right)^{1/2} - 1 +  5\epsilon d_{\max} \frac{\sum_v d_v^2 }{2\sum_v d_v^3} \le \left(5 \epsilon d_{\max} \frac{\sum_v d_v^2 }{\sum_v d_v^3}\right)^{1/2} + 2.5 \epsilon d_{\max} \frac{\sum_v d_v^2 }{\sum_v d_v^3} \\
    & \le 6\epsilon^{1/2} d_{\max} \frac{\sum_v d_v^2 }{\sum_v d_v^3}
\end{align*}

Plugging this, we get that 
\begin{align*}
        \frac{r\gamma^2 \varepsilon(Q)}{4b^2( 1 + h(5\gamma/b^2))} \ge r \varepsilon(Q)\times \epsilon^2 \frac{(\sum_v d_v^2)^2}{2m (\sum_v d_v^3)} \times (1 + 6\epsilon^{1/2} d_{\max} \frac{\sum_v d_v^2 }{\sum_v d_v^3})^{-1} \ge  r \varepsilon(Q)\times \epsilon^{3/2}\frac{(\sum_v d_v^2)}{12m d_{\max}}
\end{align*}
Setting $r = \frac{1}{\varepsilon(Q) \epsilon^{3/2}} \times \frac{12m d_{\max}}{(\sum_v d_v^2)} \log(1/\delta)$, and using Theorem~\ref{thm:lezaud}, we can claim that, with probability $1 - \delta$, 
$$ \vrw \in (1\pm \epsilon) \frac{\sum_v d_v^2}{2m}.$$
The bound on the number of nodes touched/queried by the algorithm follows naturally. 

\end{proof}

The above number of samples depends on the eigenvalue gap, $\varepsilon(Q)$, of the graph. For the specific Chung-Lu model, the value of $\varepsilon(Q)$ can be bounded by the following result from~$\cite{chung2003eigenvalues}$.

\begin{theorem}
Let $L = I - D^{-1/2}AD^{-1/2}$ denote the normalized Laplacian. Let $G$ be a random graph generated from the given expected degrees model, with expected degrees $\{\delta_i\}$, if the minimum expected degree $\delta_{\min}$ satisfies $\delta_{min} \gg \ln(n)$, then with probability at least $1-1/n= 1-o(1)$, we have that for all eigenvalues $\lambda_k(L) > \lambda_{\min}(L)$ of the 
Laplacian of $G$, 
$$\left| 1 - \lambda_k(L)\right| < 2 \sqrt{\frac{6\ln(2n)}{\delta_{\min}}} = o(1). $$
\end{theorem}

Note that $Q = D^{-1}A$ has the same set of eigenvalues as the matrix $D^{-1/2}A D^{-1/2}$. It follows above that $\varepsilon(Q) = 1 - \lambda_2(Q) = 1- \lambda_2(D^{-1/2}A D^{-1/2}) = 1 -\lambda_2(L)= 1 - o(1)$. Putting these together, we get the following corollary on the total number of node queries.
\begin{corollary}
For a graph generated from the expected degrees model, Algorithm~\ref{alg:rwestimate} 
needs to query $$\ln(n) + \frac{1}{\epsilon^{3/2}} \times \frac{12m d_{\max}}{(\sum_v d_v^2)} \log(1/\delta)$$ nodes in order to get a $(1\pm \epsilon)$ estimate of $\sum_v d_v^2/2m.$
\end{corollary}

Note $\frac{12m d_{\max}}{(\sum_v d_v^2)} \le \frac{6d_{\max}}{d_{\min}}$, but this is a loose bound, better bounds can be derived for power law degree distributions, for instance. 


\newpage
\section*{Probabilistic Guarantees (Part 5)}
We now have three competing estimators of $\lambda_1(P)$, namely:
(a) $\lambda_1(A)$,
(b) $m_2/m_1$, and 
(c) $\hat{m}_2/\hat{m}_1$.
In this section, we will establish probabilistic guarantees for the three estimators.
Note that (c) is basically the sampled version of (b).
The goal is to show that (b) (and by extension (c)) have probabilistic guarantees as strong as (a).

First, we briefly review the known probabilistic guarantees of $\lambda_1(A)$ as an estimator of $\lambda_1(P)$.
From Theorem 2.1 of~$\cite{chung2003eigenvalues}$, we know that when the condition
$$
\lambda_1^2(P) > \max_{1 \le i \le n} \delta_i \log^2(n)
$$
holds, then for any $\epsilon >0$,
$$
P[|\frac{\lambda_1(A)}{\lambda_1(P)}-1| > \epsilon]
\rightarrow 0.
$$
Our goal is to establish that similar (or stronger) guarantees for our proposed estimators, $m_2/m_1$ and 
$\hat{m}_2/\hat{m}_1$, as estimators of $\lambda_1(P)$.

Consider $m_2/m_1$.
We would like to show that under reasonable conditions, for any $\epsilon >0$,
\begin{equation}
P[|\frac{m_2/m_1}{\lambda_1(P)}-1| > \epsilon]
\rightarrow 0.
\label{m1m2_1}
\end{equation}
Recall that $\lambda_1(P) = \frac{\sum_i \delta_i^2}{\sum_i \delta_i}$.
We will show that for any $\epsilon' > 0$,
\begin{equation}
    P[|\frac{m_1}{\sum_i \delta_i} - 1| > \epsilon']
\rightarrow 0,
P[|\frac{m_2}{\sum_i \delta_i^2} - 1| > \epsilon']
\rightarrow 0.
\label{m1m2_2}
\end{equation}
We first prove that $\eqref{m1m2_2}$ implies $\eqref{m1m2_1}$.
Equation $\eqref{m1m2_2}$ implies that
$$
P[\{|\frac{m_1}{\sum_i \delta_i} - 1| > \epsilon'\} \cap \{|\frac{m_2}{\sum_i \delta_i^2} - 1| > \epsilon'\}]
\rightarrow 0.
$$
Now, consider the event
$$
\{|\frac{m_1}{\sum_i \delta_i} - 1| > \epsilon'\} \cap \{|\frac{m_2}{\sum_i \delta_i^2} - 1| > \epsilon'\}.
$$
Note that $m_2/m_1$ is a strictly increasing function of $m_2$ and a strictly decreasing function of $m_1$.
Therefore, for outcomes belonging to the above event, 
$$
\lambda_1(P) \frac{1-\epsilon'}{1+\epsilon'}
\le
\frac{m_2}{m_1}
\le
\lambda_1(P) \frac{1+\epsilon'}{1-\epsilon'}.
$$
Note that
$$
1 - \frac{1-\epsilon'}{1+\epsilon'} = 
\frac{2\epsilon'}{1+\epsilon'}
< 2\epsilon',
\text{ and }
\frac{1+\epsilon'}{1-\epsilon'}
=
\frac{2\epsilon'}{1-\epsilon'}
> \epsilon'/2,
$$
given that $\epsilon' < 1/2$.
Now, fix $\epsilon >0$ and let $\epsilon' = \epsilon/2$.
Then,
$$
\eqref{m1m2_2}
\Rightarrow
P[|\frac{m_2/m_1}{\lambda_1(P)}-1| > 2\epsilon']
\rightarrow 0
\Rightarrow
P[|\frac{m_2/m_1}{\lambda_1(P)}-1| > \epsilon]\rightarrow 0
\Rightarrow \eqref{m1m2_1}.
$$
Thus, proving \eqref{m1m2_2} is sufficient for proving \eqref{m1m2_1}.

Next, we state and prove two theorems, one on $m_1$ and one on $m_2$, which will establish \eqref{m1m2_2}.

\begin{theorem}
If the average of the expected degrees goes to infinity, i.e.,
$
\frac{1}{n}{\sum_i \delta_i} \rightarrow \infty
$,
then for any $\epsilon > 0$,
$$
P[|\frac{m_1}{\sum_i \delta_i}-1| > \epsilon] 
\rightarrow
0.
$$

\end{theorem}
\begin{proof}
We will use Hoeffding's inequality \citep{hoeffding1994probability}, and we begin by stating the inequality for the sum of Bernoulli random variables.
Let $B_1, \ldots, B_m$ be $m$ independent (but not necessarily identically distributed) Bernoulli random variables, and $S_m = \sum_{i=1}^m B_i$.
Then for any $t > 0$,
$$
P[|S_m - {E}[S_m]| \geq t]
\le 
2 \exp\left({\frac{-2t^2}{m}}\right).
$$
In our case, 
$$
m_1 = \sum_{i=1}^n d_i
= \sum_{i=1}^n \sum_{j=1}^n A(i,j)
= 2 \sum_{i<j} A(i,j),
$$
and we know that $\{A(i,j): 1 \le i < j \le n\}$ are independent Bernoulli random variables. 
Fix $\epsilon > 0$ and note that $E[\sum_{i<j} A(i,j)] = \frac{1}{2}\sum_i \delta_i$.
Using Hoeffding's inequality with $S_m = m_1/2$, $m = {n \choose 2}$, and $t = \frac{\epsilon}{2} \sum_i \delta_i$,
we get
$$
P[|\frac{m_1}{2} - \frac{\sum_i \delta_i}{2}| >
\frac{\epsilon}{2} \sum_i \delta_i]
\le
2 \exp\left(-\epsilon^2
{\frac{(\sum_i \delta_i)^2}{n(n-1)}}\right).
$$
Since $
\frac{1}{n}{\sum_i \delta_i} \rightarrow \infty
$, the right hand side goes to zero.
Therefore,
$$
P[|\frac{m_1}{\sum_i \delta_i} -1| >
\epsilon]
\rightarrow
0.
$$
\end{proof}

